Alleviating the Burden of Labeling: Sentence Generation by Attention Branch Encoder-Decoder Network

Domestic service robots (DSRs) are a promising solution to the shortage of home care workers. However, one of the main limitations of DSRs is their inability to interact naturally through language. Recently, data-driven approaches have been shown to be effective for tackling this limitation; however, they often require large-scale datasets, which is costly. Based on this background, we aim to perform automatic sentence generation of fetching instructions: for example, "Bring me a green tea bottle on the table." This is particularly challenging because appropriate expressions depend on the target object, as well as its surroundings. In this paper, we propose the attention branch encoder--decoder network (ABEN), to generate sentences from visual inputs. Unlike other approaches, the ABEN has multimodal attention branches that use subword-level attention and generate sentences based on subword embeddings. In experiments, we compared the ABEN with a baseline method using four standard metrics in image captioning. Results show that the ABEN outperformed the baseline in terms of these metrics.

==> section5_dataset.tex <==

\section{Dataset
\label{dataset}
}
% \subsection{Dataset construction overview}
% The dataset was collected from a simulated home environment as described in Section ??. The environment setup is described as follow
% \begin{itemize}
% \item The robot is beforehand placed in front of a randomly selected destination at a reachable distance.
% \item The robot holds a randomly selected target to place on the selected destination.
% \item  The destination is cluttered by a random number of obstacles. 
% \end{itemize}

% The procedure given below describes the different steps used to build the carry-and-place multi-modal data set. Each of these steps will be detailed in the following sections.
% \begin{itemize}
% \item[$1$.] Setup an area with everyday objects as described above.
% \item[$2$.] Record the scene with the robot embedded cameras (RGB and depth).
% \item[$3$.] Place the target on the destination.
% \item[$4$.] Record the collision statistics.
% \end{itemize} 

% \subsection{Environment setup}
% Using a simulated environment, allow us to collect a large-scale data in several configurations through an automated process. It is important to have  variation in the dataset to be able to generalize PonNet and ensure that it does not overfit to a predefined scene setting or configuration. As depicted in Fig.\ref{fig:env_setup}, the simulated environment is a procedural home environment composed of a kitchen, living room, bedroom and lobby. For more variety, we considered twelve different locations distributed among these rooms to perform the placing task. As so, the data was collected with different background and lighting conditions. 

% For each location, a DSR was placed in front of a given destination. A destination correspond to daily furniture such as tables shelves, sofas, etc. Each of them has a different shape, material and reflection property. A set of six destination candidates was considered. For each task, a randomly sampled destination is selected. It should be noted, that destinations like shelves have two levels that could be selected as placing area.

% Before performing the placing task, obstacles are scattered on each destination. These obstacles refer to daily objects in the environment. A set of 28 objects was considered. The number of obstacle on a given destination is random varying from none to 20. To increase the variation of obstacle position and orientation, all obstacles are dropped on the destination from a given height. 

% Similarly to obstacles, the target is an object selected among a set of 15 daily objects that are graspable by a DSR. The target is supposedly hold by the robot. 

% \begin{figure}[t]
% \subfloat{\includegraphics[width=0.485\columnwidth]{fig/environment1.png}} \enskip
% \subfloat{\includegraphics[width=0.485\columnwidth]{fig/environment2.png}} \\\vskip -10pt
% \subfloat{\includegraphics[width=0.485\columnwidth, height=3cm]{fig/destinations.png}}\enskip
% \subfloat{\includegraphics[width=0.485\columnwidth, height=3cm]{fig/obstacles.png}}
% \caption{\small Simulator environment setup. Top-row figures show the placing task in different conditions. Bottom-row figures illustrate samples of the destinations and objects used as obstacles or targets.}
% \label{fig:env_setup}
% \centering
% \end{figure}

% \subsection{Placing task}
% As the environment is setup, the robot recorded through RGB and depth modality the state of the destination with head-mounted cameras as 480 $\times$ 640 images. Additionally, the destination height and the target dimension were also recorded. Thereafter, the robot could perform the placing task (please refer to the accompanying video) by extending its arm. The collision statistics were then recorded for each task. As our focus is on the prediction of damaging collision, no placing strategy nor obstacle avoidance were implemented. Similarly the simulator does not handle slip and friction. These parameters are out of the scope of this paper.

% \subsection{Labeling Strategy}
% Each placing task was then automatically labeled from the simulator. Two labels, $A1$ and $A2$, were used to define the success or failure of the placing task. A placing task was considered successful if it did not generate any damaging collision. In this case, this placing task was labeled $A1$, otherwise the label $A2$ was given. A damaging collision is defined as any collision involving the robot, target, obstacles or destination with a speed  greater than 0.1 m/s.  From the simulator four types of damaging collisions can be characterized:
% \begin{itemize}
% \item collisions between the robot arm and some obstacles,
% \item collisions between the robot and the target destination,
% \item collisions between several obstacles,
% \item collisions between the target and some obstacles.
% \end{itemize}
% Hence, from the characteristics of damaging collisions, predicting the outcome of a placing task becomes challenging. Indeed, for instance,  a plain motion that slightly touches some obstacles with a speed below 0.1 m/s is labelled as a successful $A1$. Using the robot 3D model or detecting free areas does not allow to predict accurately such cases, as damaging collisions highly depend on the physics of the objects interacting in the environment. 

% From the environment setup and the labeling strategy described above, we could collect 12,000 samples (1,000 samples for each location). This dataset was randomly split into training (10,000 samples), validation (1,000 samples) and test (1,000 samples) sets. After removing the invalid samples, we could obtained the dataset summarized in Table \ref{tab:dataset}.




% \begin{table}[h]
% \normalsize
% \caption{\small Statistics of PonNet dataset}
% \label{tab:dataset}
% \centering
% \begin{tabular}{cccc|c }
% \hline
% $\#$ & Train& Valid.& Test& $\sum$\\
% \hline
% $A1$&4807&492&448&{\bf 5747} \\

% $A2$&5074&496&490&{\bf 6060}\\
% \hline
% $\sum$& {\bf 9881}  & {\bf 988} & {\bf 938}  & \multicolumn{1}{ |c}{\bf 11807}\\
% $\%$ &83.7&8.4 &7.9&100\\
% \hline
% \end{tabular}
% \end{table}


% \begin{figure}[ht]
% \begin{subfigure}{0.45\textwidth}
% \includegraphics[width=0.3\linewidth, height=2cm]{fig/scoring/0003_rgb.jpg} 
% \includegraphics[width=0.3\linewidth, height=2cm]{fig/scoring/0003_rgb.jpg}
% \includegraphics[width=0.3\linewidth, height=2cm]{fig/scoring/0003_rgb.jpg}
% \caption{Success}
% \label{fig:success}
% \end{subfigure}

% \begin{subfigure}{0.45\textwidth}
% \includegraphics[width=0.3\linewidth, height=2cm]{fig/scoring/0003_rgb.jpg} 
% \includegraphics[width=0.3\linewidth, height=2cm]{fig/scoring/0003_rgb.jpg}
% \includegraphics[width=0.3\linewidth, height=2cm]{fig/scoring/0003_rgb.jpg}
% \caption{Failure}
% \label{fig:fail}
% \end{subfigure}

% \caption{Scoring and labeling samples(mock images)}
% \label{fig:scoring}
% \end{figure}





% Local Variables:
% eval: (auto-fill-mode -1)
% coding: utf-8
% End:

